MPC-guided, Data-driven Fuzzy Controller Synthesis

Model predictive control (MPC) is a powerful control technique for online optimization using system model-based predictions over a finite time horizon. However, the computational cost MPC requires can be prohibitive in resource-constrained computer systems. This paper presents a fuzzy controller synthesis framework guided by MPC. In the proposed framework, training data is obtained from MPC closed-loop simulations and is used to optimize a low computational complexity controller to emulate the response of MPC. In particular, autoregressive moving average (ARMA) controllers are trained using data obtained from MPC closed-loop simulations, such that each ARMA controller emulates the response of the MPC controller under particular desired conditions. Using a Takagi-Sugeno (T-S) fuzzy system, the responses of all the trained ARMA controllers are then weighted depending on the measured system conditions, resulting in the Fuzzy-Autoregressive Moving Average (F-ARMA) controller. The effectiveness of the trained F-ARMA controllers is illustrated via numerical examples.

==> PackagesCommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb}  % assumes amsmath package installed
\usepackage{amsfonts}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}[section]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
% % \newtheorem{definitionSec}{Definition}[subsection]
\newtheorem{exmp}{Example}[section]
% \newtheorem{exmpSec}{Example}[subsection]
\newtheorem{fact}{Fact}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{factSec}{Fact}[subsection]
% \newtheorem{theorem}{Theorem}[section]
\newtheorem{problem}{Problem}[section]
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}[section]


% \newtheorem{prob}{Problem}[section]
\newtheorem{prob}{Problem}

% \usepackage{graphicx}
% \usepackage{epsfig}
% \usepackage{epstopdf}
% \usepackage{math tools}
% \usepackage{color}
% \usepackage[utf8]{inputenc}
%\pagestyle{plain}

% \usepackage{subfigure}
% \usepackage{subfig}
\usepackage{float} 
\usepackage[skip=0em,font=footnotesize]{caption}
% \usepackage{wrapfig}%   wrap figures/tables in text (i.e., Di Vinci style)
% \usepackage[export]{adjustbox}

% \usepackage{geometry}
% \usepackage{indentfirst}


% \usepackage{epsfig} % for postscript graphics files

% \usepackage{lastpage}
% \usepackage{fancyhdr}
% \pagestyle{fancy} 
% \cfoot{\thepage\ of \pageref{LastPage}}
% \fancyhead{}
% \renewcommand{\headrulewidth}{0pt}

% \usepackage{mathptmx} % assumes new font selection scheme installed
% \usepackage{times} % assumes new font selection scheme installed


% \usepackage[mathscr]{euscript}

% \usepackage{newtxtext}
% \usepackage{newtxmath}

% \usepackage{subfiles}
% \usepackage{cancel}
% \usepackage{imakeidx}

%\usepackage{citesort}
%\usepackage[fleqn]{amsmath}
%\usepackage{fullpage}
%\usepackage[top=0.75in,bottom= 0.75in,left = 0.75in, right = 0.75in]{geometry}
\usepackage[margin = 1in]{geometry}

%\parskip = -0.5pt
%\parindent = 2pt %0in


%\usepackage{multicol}
%\usepackage{caption}
%\usepackage[skip=2pt]{caption}
%\usepackage[skip=1pt,font=footnotesize]{caption}
%\usepackage[skip=1pt,font=small]{caption}
%\usepackage{subcaption}






\usepackage{tikz}
\usetikzlibrary{shapes,arrows,calc,positioning}
\tikzstyle{bigblock} = [draw, fill=blue!20, rectangle, 
    minimum height=6em, minimum width=8em]
\tikzstyle{medblock} = [draw, fill=blue!20, rectangle, 
    minimum height=4em, minimum width=4em]    
\tikzstyle{mux} = [draw, fill=black!20, rectangle, 
    minimum height=5em, minimum width=0.1em]    
\tikzstyle{smallblock} = [draw, fill=blue!20, rectangle, 
    minimum height=2em, minimum width=3em]
    
\tikzstyle{data_block} = [draw, fill=green!20, rectangle, 
    minimum height=2em, minimum width=3em]
\tikzstyle{ops_block} = [draw, fill=blue!20, rectangle, 
    minimum height=2em, minimum width=3em]    
\tikzstyle{est_block} = [draw, fill=red!20, rectangle, 
    minimum height=2em, minimum width=3em]    
    
\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm,minimum height=0.5cm]
\tikzstyle{signal} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{block} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=9em]
\tikzstyle{blockS} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=4em]    
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\usetikzlibrary{matrix}

\usetikzlibrary{positioning}
\usetikzlibrary{math} 



\usepackage{hyperref}
\usepackage{xcolor}
\hypersetup{
    colorlinks,
    linkcolor={blue!100!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}

% \usepackage{diagbox}


%\newtheorem{definition}{Definition}[section]
%\usepackage{biblatex}
% \addbibresource{mendeley_v2.bib}

% \usepackage[square, numbers, sort&compress]{natbib} 
% \setcitestyle{square braces, numbers}
%\usepackage{cite}



%\usepackage[nomarkers,figuresonly]{endfloat}

% \renewcommand{\familydefault}{\rmdefault}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% COMMANDS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\nn}{\nonumber}
\newcommand{\matl}{\left[ \begin{array}}
\newcommand{\matr}{\end{array} \right]}

\renewcommand{\matl}{\begin{bmatrix}}
\renewcommand{\matr}{\end{bmatrix}}

\newcommand{\matls}{\left[ \begin{smallmatrix}}
\newcommand{\matrs}{\end{smallmatrix} \right]}
\newcommand{\isdef}{\stackrel{\triangle}{=}}
\newcommand{\pr}[1]{{#1}^{\prime}}
\newcommand{\inv}{^{-1}}
\newcommand{\row}[1]{{\rm row}_{#1}}
\newcommand{\col}[1]{{\rm col}_{#1}}
\newcommand{\arrowup}[1]{\stackrel{#1}{\SLeftarrow}}
\newcommand{\smin}{\stackrel{\min}{\sim}}
\newcommand{\jw}{\jmath \omega}
\newcommand{\omegan}{\omega_{\rm n}}
\newcommand{\omegad}{\omega_{\rm d}}
\newcommand{\omegar}{\omega_{\rm r}}
\newcommand{\omegani}{\omega_{{\rm n}i}}
\newcommand{\omegans}[1]{\omega_{{\rm n}_{#1}}}
\newcommand{\MSig}{{\mit\Sigma}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\vect}[1]{\overset{\rightharpoonup}{#1}}
\newcommand{\HS}{\hat S}
\newcommand{\HI}{\hat I}
\newcommand{\rmThat}{{\hat{\rm T}}}
\newcommand{\asthat}{{\hat*}}
\newcommand{\dpder}[2]{\displaystyle\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\der}[2]{\mbox{$\frac{d{#1}}{d{#2}}$}}
\newcommand{\dder}[2]{\displaystyle{\frac{d{#1}}{d{#2}}}}
\newcommand{\pder}[2]{\mbox{$\frac{\partial {#1}}{\partial {#2}}$}}
\newcommand{\dt}{{\rm d}t}
\newcommand{\dx}{{\rm d}x}
\newcommand{\p}{\partial}
\newcommand{\pt}{\partial_t}
\newcommand{\ptt}{\partial^2_t}
\newcommand{\px}{\partial_x}
\newcommand{\pxx}{\partial^2_x}
\newcommand{\pp}{\partial{^2}}
\newcommand{\tr}{{\rm tr}\,}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\DeclareMathOperator{\tr}{tr}
\newcommand{\rmA}{{\rm A}}
\newcommand{\rmB}{{\rm B}}
\newcommand{\rmC}{{\rm C}}
\newcommand{\rmD}{{\rm D}}
\newcommand{\rmE}{{\rm E}}
\newcommand{\rmF}{{\rm F}}
\newcommand{\rmG}{{\rm G}}
\newcommand{\rmH}{{\rm H}}
\newcommand{\rmI}{{\rm I}}
\newcommand{\rmJ}{{\rm J}}
\newcommand{\rmK}{{\rm K}}
\newcommand{\rmL}{{\rm L}}
\newcommand{\rmM}{{\rm M}}
\newcommand{\rmN}{{\rm N}}
\newcommand{\rmO}{{\rm O}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmQ}{{\rm Q}}
\newcommand{\rmR}{{\rm R}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmU}{{\rm U}}
\newcommand{\rmV}{{\rm V}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\rmX}{{\rm X}}
\newcommand{\rmY}{{\rm Y}}
\newcommand{\rmZ}{{\rm Z}}
\newcommand{\rma}{{\rm a}}
\newcommand{\rmb}{{\rm b}}
\newcommand{\rmc}{{\rm c}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\rme}{{\rm e}}
\newcommand{\rmf}{{\rm f}}
\newcommand{\rmg}{{\rm g}}
\newcommand{\rmh}{{\rm h}}
\newcommand{\rmi}{{\rm i}}
\newcommand{\rmj}{{\rm j}}
\newcommand{\rmk}{{\rm k}}
\newcommand{\rml}{{\rm l}}
\newcommand{\rmm}{{\rm m}}
\newcommand{\rmn}{{\rm n}}
\newcommand{\rmo}{{\rm o}}
\newcommand{\rmp}{{\rm p}}
\newcommand{\rmq}{{\rm q}}
\newcommand{\rmr}{{\rm r}}
\newcommand{\rms}{{\rm s}}
\newcommand{\rmt}{{\rm t}}
\newcommand{\rmu}{{\rm u}}
\newcommand{\rmv}{{\rm v}}
\newcommand{\rmw}{{\rm w}}
\newcommand{\rmx}{{\rm x}}
\newcommand{\rmy}{{\rm y}}
\newcommand{\rmz}{{\rm z}}
\newcommand{\BBA}{{\mathbb A}}
\newcommand{\BBB}{{\mathbb B}}
\newcommand{\BBC}{{\mathbb C}}
\newcommand{\BBD}{{\mathbb D}}
\newcommand{\BBE}{{\mathbb E}}
\newcommand{\BBF}{{\mathbb F}}
\newcommand{\BBG}{{\mathbb G}}
\newcommand{\BBH}{{\mathbb H}}
\newcommand{\BBI}{{\mathbb I}}
\newcommand{\BBJ}{{\mathbb J}}
\newcommand{\BBK}{{\mathbb K}}
\newcommand{\BBL}{{\mathbb L}}
\newcommand{\BBM}{{\mathbb M}}
\newcommand{\BBN}{{\mathbb N}}
\newcommand{\BBO}{{\mathbb O}}
\newcommand{\BBP}{{\mathbb P}}
\newcommand{\BBQ}{{\mathbb Q}}
\newcommand{\BBR}{{\mathbb R}}
\newcommand{\BBS}{{\mathbb S}}
\newcommand{\BBT}{{\mathbb T}}
\newcommand{\BBU}{{\mathbb U}}
\newcommand{\BBV}{{\mathbb V}}
\newcommand{\BBW}{{\mathbb W}}
\newcommand{\BBX}{{\mathbb X}}
\newcommand{\BBY}{{\mathbb Y}}
\newcommand{\BBZ}{{\mathbb Z}}

\newcommand{\real}{{\mathbb{R}}}
\newcommand{\comp}{{\mathbb{C}}}
\newcommand{\realR}{\mathbb{R}}

\newcommand{\SA}{{\mathcal A}}
\newcommand{\SB}{{\mathcal B}}
\newcommand{\SC}{{\mathcal C}}
\newcommand{\SD}{{\mathcal D}}
\newcommand{\SE}{{\mathcal E}}
\newcommand{\SF}{{\mathcal F}}
\newcommand{\SG}{{\mathcal G}}
\newcommand{\SH}{{\mathcal H}}
% \newcommand{\SI}{{\mathcal I}}
\newcommand{\SJ}{{\mathcal J}}
\newcommand{\SK}{{\mathcal K}}
\newcommand{\SL}{{\mathcal L}}
\newcommand{\SM}{{\mathcal M}}
\newcommand{\SN}{{\mathcal N}}
\newcommand{\SO}{{\mathcal O}}
\newcommand{\SP}{{\mathcal P}}
\newcommand{\SQ}{{\mathcal Q}}
\newcommand{\SR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\ST}{{\mathcal T}}
\newcommand{\SU}{{\mathcal U}}
\newcommand{\SV}{{\mathcal V}}
\newcommand{\SW}{{\mathcal W}}
\newcommand{\SX}{{\mathcal X}}
\newcommand{\SY}{{\mathcal Y}}
\newcommand{\SZ}{{\mathcal Z}}
\newcommand{\BFA}{{\bf A}}
\newcommand{\BFB}{{\bf B}}
\newcommand{\BFC}{{\bf C}}
\newcommand{\BFD}{{\bf D}}
\newcommand{\BFE}{{\bf E}}
\newcommand{\BFF}{{\bf F}}
\newcommand{\BFG}{{\bf G}}
\newcommand{\BFH}{{\bf H}}
\newcommand{\BFI}{{\bf I}}
\newcommand{\BFJ}{{\bf J}}
\newcommand{\BFK}{{\bf K}}
\newcommand{\BFL}{{\bf L}}
\newcommand{\BFM}{{\bf M}}
\newcommand{\BFN}{{\bf N}}
\newcommand{\BFO}{{\bf O}}
\newcommand{\BFP}{{\bf P}}
\newcommand{\BFQ}{{\bf Q}}
\newcommand{\BFR}{{\bf R}}
\newcommand{\BFS}{{\bf S}}
\newcommand{\BFT}{{\bf T}}
\newcommand{\BFU}{{\bf U}}
\newcommand{\BFV}{{\bf V}}
\newcommand{\BFW}{{\bf W}}
\newcommand{\BFX}{{\bf X}}
\newcommand{\BFY}{{\bf Y}}
\newcommand{\BFZ}{{\bf Z}}
\def\bbR{\mbox{\bbfnt R}}
\newcommand{\vspaceAnkit}{\vspace{-3pt}}
\newcommand{\shiftq}{{\textbf{\textrm{q}}}}








% \newtheoremstyle{factindented}
%     {3pt}
%     {3pt}
%     {\addtolength{\leftskip}{1.5em}}
%     {}
%     {\bfseries}
%     {.}
%     {.5em}
%     {}
% %\theoremstyle{factindented}


% \newtheoremstyle{indented}
%     {3pt}
%     {3pt}
%     {\addtolength{\leftskip}{3em}}
%     {}
%     {\bfseries}
%     {.}
%     {.5em}
%     {}

% \theoremstyle{indented}







% \newcommand{\SCA}{{\mathscr{A}}}
% \newcommand{\SCB}{{\mathscr{B}}}
% \newcommand{\SCU}{{\mathscr{U}}}

\newcommand{\Star}{^{*}}

%\newcommand{\scM}{{\mathscr M}}
\newcommand{\scM}{{\mathcal M}}

\newcommand{\neweqline}{\ensuremath{\nn \\ &\quad }}

\newcommand{\framedot}[2]{\stackrel{{\rm #1}\bullet}{#2}}
\newcommand{\frameddot}[2]{\stackrel{{\rm #1}\bullet \bullet}{#2}}

\newcommand{\polar}[1]{\ensuremath{r_{#1}e^{\jmath \theta_{#1}}}}

\newcommand{\tarrow}[1]{\overset{\rightarrow}{#1}}


%% to do list functions
\usepackage{enumitem,amssymb}
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}
\newcommand{\inprogress}{\rlap{$\square$}{\large\hspace{1pt}\ding{45}}}

